OASIS-ERIS: Open Acquisition System for IEPE Sensors - Electrically Refined and Inter-device Synchronization

OASIS-ERIS, the Open Acquisition System for IEPE Sensors - Electrically Refined and Inter-device Synchronization, is the successor to the previously released OASIS-UROS. It is based on the Analog Devices AD7606C-18 analog-to-digital converter, offering 18-bit resolution on eight simultaneously sampled channels, and the Espressif ESP32-S3 microcontroller. The laboratory usability of OASIS-ERIS is significantly improved compared to OASIS-UROS due to the added inter-device synchronization. By physically connecting the sample clocks across devices, a truly synchronized data acquisition can be achieved with an arbitrary number of acquisition boards. Additionally, a migration of the firmware to ESP-IDF allows a major increase of the achievable sampling frequency to 100 kHz. This paper documents the hardware and software stack of OASIS-ERIS, and provides all materials necessary for reproduction. Further, the performance of OASIS-ERIS is tested against a commercial measurement system in an Experimental Modal Analysis campaign. The results show that OASIS-ERIS closely matches the performance of the commercial system, making it a viable replacement for academia and projects with tightly constrained budgets.

==> source/statements.tex <==
% !TeX spellcheck = en_US

\paragraph{CRediT authorship contribution statement} 
\textbf{O.~M.~Zobel:} Conceptualization; Data curation; Formal analysis; Funding acquisition; Investigation; Methodology; Project administration; Resources; Software; Supervision; Validation; Visualization; Writing – original draft; Writing – review \& editing. 
\textbf{S.~Author:} Existence. 

\paragraph{Data availability}
The ... are available at: \url{https://doi.org/XX.XXXXX/XXXXXXXXXXXXXX}, \cite{Data}.

\paragraph{Declaration of Competing Interest} 
The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work reported in this paper.

\paragraph{Funding}
This work was supported by \textit{SUPPORTING COMPANY}.
